Influence-Driven Explanations for Bayesian Network Classifiers

One of the most pressing issues in AI in recent years has been the need to address the lack of explainability of many of its models. We focus on explanations for discrete Bayesian network classifiers (BCs), targeting greater transparency of their inner workings by including intermediate variables in explanations, rather than just the input and output variables as is standard practice. The proposed influence-driven explanations (IDXs) for BCs are systematically generated using the causal relationships between variables within the BC, called influences, which are then categorised by logical requirements, called relation properties, according to their behaviour. These relation properties both provide guarantees beyond heuristic explanation methods and allow the information underpinning an explanation to be tailored to a particular context's and user's requirements, e.g., IDXs may be dialectical or counterfactual. We demonstrate IDXs' capability to explain various forms of BCs, e.g., naive or multi-label, binary or categorical, and also integrate recent approaches to explanations for BCs from the literature. We evaluate IDXs with theoretical and empirical analyses, demonstrating their considerable advantages when compared with existing explanation methods.

==> 2020 - ArXiv - IDX/tables/datasets.tex <==
\begin{tabular}{r|cc|cc|cc|cc}
  \multirow{ 2}{*}{\!\!Dataset\!\!} & 
  \multirow{ 2}{*}{\!\!\!BC$^{\dagger}$\!\!\!} & 
  \multirow{ 2}{*}{\!\!Size\!\!} & 
  \multicolumn{2}{c}{\!\!Variables\!\!} &
  \multicolumn{2}{c}{\!\!Types$^{\ddagger}$\!\!} & 
  \multicolumn{2}{c}{\!\!Performance$^{\mathsection}$\!\!}\\
  & & & \!\!$|\Obs|$\!\! & \!\!$|\Cla|$\!\! & \!\!$\Obs$\!\! & \!\!$\Cla$\!\! &\!\!Accuracy\!\!& \!\!F1\!\!\\
\hline
%  \!\!\textbf{Play}$^*$ & \!\!BCC\!\! & \!\!16\!\! & \!\!4\!\! & \!\!2\!\! & \!\!B\!\! & \!\!B\!\! & \!\!100.0\%\!\! & \!\!1.00\!\!\\
 \!\!\textbf{Shuttle}\tablefootnote{\label{footnote:UCI}Machine Learning Repository \cite{UCIDatasets}} & \!\!NBC\!\! & \!\!278\!\! & \!\!6\!\! & \!\!1\!\! & \!\!C\!\! & \!\!B\!\! & \!\!95.7\%\!\! & \!\!0.96\!\!\\
 \!\!\textbf{Votes}%\footnotemark[
 \textsuperscript{\ref{footnote:UCI}}
 %] 
 & \!\!NBC\!\! & \!\!435\!\! & \!\!16\!\! & \!\!1\!\! & \!\!B\!\! & \!\!B\!\! & \!\!90.8\%\!\! & \!\!0.90\!\!\\
 \!\!\textbf{Parole}\tablefootnote{National Archive of Criminal Justice Data \cite{ParoleDataset}} & \!\!NBC\!\! & \!\!675\!\! & \!\!8\!\! & \!\!1\!\! & \!\!C\!\! & \!\!B\!\! & \!\!88.8\%\!\! & \!\!0.69\!\!\\
 \!\!\textbf{German}%\footnotemark[
 \textsuperscript{\ref{footnote:UCI}}%]
 & \!\!NBC\!\! & \!\!750\!\! & \!\!20\!\! & \!\!1\!\! & \!\!C\!\! & \!\!B\!\! & \!\!76.4\%\!\! & \!\!0.72\!\!\\
 \!\!\textbf{COMPAS}\tablefootnote{ProRepublica Data Store \cite{COMPASDataset}} & \!\!NBC\!\! & \!\!6951\!\! & \!\!12\!\! & \!\!1\!\! & \!\!C\!\! & \!\!B\!\! & \!\!70.5\%\!\! & \!\!0.71\!\!\\
 \!\!\textbf{Car}%\footnotemark[
 \textsuperscript{\ref{footnote:UCI}}
 %] 
 & \!\!NBC\!\! & \!\!1728\!\! & \!\!6\!\! & \!\!1\!\! & \!\!C\!\! & \!\!C\!\! & \!\!86.6\%\!\! & \!\!0.76\!\!\\
 \!\!\textbf{Emotions}\tablefootnote{Multi-Label Classification Dataset Repository \cite{UCODatasets}} & \!\!BCC\!\! & \!\!593\!\! & \!\!72\!\! & \!\!6\!\! & \!\!C\!\! & \!\!B\!\! & \!\!80.2\%\!\! & \!\!0.70\!\!\\
  \!\!\textbf{Asia}\tablefootnote{\label{footnote:bnlearn}Bayesian Network Repository \cite{BNLearnDatasets}} & \!\!BCC\!\! & \!\!4\!\! & \!\!2\!\! & \!\!6\!\! & \!\!B\!\! & \!\!B\!\! & \!\!100\%\!\! & \!\!1.00\!\!\\
 \!\!\textbf{Child}%\footnotemark[
 \textsuperscript{\ref{footnote:bnlearn}}
 %] 
 & \!\!BCC\!\! & \!\!1080\!\! & \!\!7\!\! & \!\!13\!\! & \!\!C\!\! & \!\!C\!\! & \!\!80.6\%\!\! & \!\!0.66\!\!\\
\end{tabular}

==> 2020 - ArXiv - IDX/tables/monotonicity.tex <==
\begin{tabular}{r|c|c|c}
Dataset & SM-IDX & LIME-IDX & SHAP-IDX\\
\hline
\textbf{Shuttle}  &   \!\!5.8\%\!\! &   \!\!6.8\%\!\! &   \!\!6.5\%\!\! \\
\textbf{Votes}    &   \!\!0.0\%\!\! &   \!\!0.2\%\!\! &   \!\!0.1\%\!\! \\
\textbf{Parole}   &  \!\!13.3\%\!\! &  \!\!13.2\%\!\! &  \!\!13.8\%\!\! \\
\textbf{German}   &  \!\!18.5\%\!\! &  \!\!20.8\%\!\! &  \!\!19.8\%\!\! \\
\textbf{COMPAS}   &  \!\!12.3\%\!\! &  \!\!12.5\%\!\! &  \!\!22.7\%\!\! \\
\textbf{Car}      &  \!\!16.8\%\!\! &  \!\!18.5\%\!\! &  \!\!17.4\%\!\! \\
\textbf{Emotions} &  \!\!12.0\%\!\! &  \!\!11.9\%\!\! &   \!\!8.9\%\!\! \\
\textbf{Child}    &   \!\!7.1\%\!\! &   \!\!2.5\%\!\! &   \!\!5.6\%\!\! \\
\textbf{Asia}     &   \!\!0.0\%\!\! &   \!\!0.0\%\!\! &   \!\!0.0\%\!\! \\

\end{tabular}

==> 2020 - ArXiv - IDX/tables/old/play.tex <==
\begin{tabular}{ccccccccc}
\hline
	\multicolumn{5}{c}{\!\!$\SF$\!\!} & \multicolumn{2}{c}{SD-IDX} & %\multicolumn{2}{c}{SD-IDX} & 
	\multicolumn{2}{c}{CF-IDX}  \\
%\cline{1-5}
%\cline{8-8}
\!\!\!$w$\!\!\! & 
\!\!\!$t$\!\!\! & 
%\!\!\!$h$\!\!\! & 
\!\!\!$p$\!\!\! & 
\!\!\!$r$\!\!\! & 
\!\!\!$o$\!\!\! & 
%\!\!$\SDAtts\!(\!r\!)$/$\SDSupps\!(\!r\!)$\!\!\!\! &
\!\!$\dot{-}(\!r\!)$/$\dot{+}(\!r\!)$\!\!\!\! &
\!\!\!$\dot{-}(\!o\!)$/$\dot{+}(\!o\!)$\!\!\! &
\!\!\!$!(\!r\!)$/$*(\!r\!)$\!\!\!\! &
\!\!\!\!$!(\!o\!)$/$*(\!o\!)$\!\!\! \\
\hline
%
\!\!\!$l$\!\!\! & 
\!\!\!$l$\!\!\! & 
\!\!\!$l$\!\!\! & 
\!\!\!$+$\!\!\! & 
\!\!\!$-$\!\!\! &
$\{ t \}$/$\{ \textit{\textbf{p}} \}$ &
$\{ \textit{\textbf{w}} \}$/$\{ t, \textit{\textbf{r}}  \}$ &
$\{ p \}$/$\{  \}$ &
$\{ r \}$/$\{ t \}$ \\
%
\!\!\!$m$\!\!\! & 
\!\!\!$l$\!\!\! & 
\!\!\!$l$\!\!\! & 
\!\!\!$+$\!\!\! & 
\!\!\!$-$\!\!\! &
$\{ t \}$/$\{ \textit{\textbf{p}} \}$ &
\!\!\!$\{  \}$/$\{ w, t, \textit{\textbf{r}} \}$\!\!\! &
$\{ p \}$/$\{  \}$ &
\!\!\!$\{  \}$/$\{ w, t, r \}$\!\!\! \\
%
\!\!\!$l$\!\!\! & 
\!\!\!$m$\!\!\! & 
\!\!\!$l$\!\!\! & 
\!\!\!$+$\!\!\! & 
\!\!\!$-$\!\!\! &
$\{ t \}$/$\{ \textit{\textbf{p}} \}$ &
$\{ \textit{\textbf{w}}, \textit{\textbf{t}} \}$/$\{ \textit{\textbf{r}} \}$ &
$\{ p \}$/$\{  \}$ &
$\{ r \}$/$\{  \}$ \\
%
\!\!\!$m$\!\!\! & 
\!\!\!$m$\!\!\! & 
\!\!\!$l$\!\!\! & 
\!\!\!$+$\!\!\! & 
\!\!\!$-$\!\!\! &
$\{ t \}$/$\{ \textit{\textbf{p}} \}$ &
$\{ \textit{\textbf{t}} \}$/$\{  w, \textit{\textbf{r}} \}$ &
$\{ p \}$/$\{  \}$ &
$\{ r \}$/$\{ w \}$ \\
%
\!\!\!$h$\!\!\! & 
\!\!\!$l$\!\!\! & 
\!\!\!$l$\!\!\! & 
\!\!\!$+$\!\!\! & 
\!\!\!$-$\!\!\! &
$\{ t \}$/$\{ \textit{\textbf{p}} \}$ &
\!\!\!$\{  \}$/$\{ w, t, \textit{\textbf{r}} \}$\!\!\! &
$\{ p \}$/$\{  \}$ &
\!\!\!$\{  \}$/$\{ w, t, r \}$\!\!\! \\
%
\!\!\!$l$\!\!\! & 
\!\!\!$h$\!\!\! & 
\!\!\!$l$\!\!\! & 
\!\!\!$+$\!\!\! & 
\!\!\!$-$\!\!\! &
$\{  \}$/$\{ \textit{\textbf{t}}, \textit{\textbf{p}} \}$ &
$\{ \textit{\textbf{w}} \}$/$\{ \textit{\textbf{t}}, \textit{\textbf{r}} \}$ &
$\{  \}$/$\{ t, p \}$ &
$\{  \}$/$\{ r \}$ \\
%
\!\!\!$h$\!\!\! & 
\!\!\!$m$\!\!\! & 
\!\!\!$l$\!\!\! & 
\!\!\!$+$\!\!\! & 
\!\!\!$-$\!\!\! &
$\{ t \}$/$\{ \textit{\textbf{p}} \}$ &
$\{ \textit{\textbf{t}} \}$/$\{ w, \textit{\textbf{r}} \}$ &
$\{ p \}$/$\{  \}$ &
$\{ r \}$/$\{ w \}$ \\
%
\!\!\!$m$\!\!\! & 
\!\!\!$h$\!\!\! & 
\!\!\!$l$\!\!\! & 
\!\!\!$+$\!\!\! & 
\!\!\!$-$\!\!\! &
$\{  \}$/$\{ \textit{\textbf{t}}, \textit{\textbf{p}} \}$ &
\!\!\!$\{  \}$/$\{ w, \textit{\textbf{t}}, \textit{\textbf{r}} \}$\!\!\! &
$\{  \}$/$\{ t, p \}$ &
$\{  \}$/$\{ w, r \}$ \\
%
\!\!\!$h$\!\!\! & 
\!\!\!$h$\!\!\! & 
\!\!\!$l$\!\!\! & 
\!\!\!$+$\!\!\! & 
\!\!\!$-$\!\!\! &
$\{  \}$/$\{ \textit{\textbf{t}}, \textit{\textbf{p}} \}$ &
\!\!\!$\{  \}$/$\{ w, \textit{\textbf{t}}, \textit{\textbf{r}} \}$\!\!\! &
$\{  \}$/$\{ t, p \}$ &
$\{  \}$/$\{ w, r \}$ \\
%
\!\!\!$l$\!\!\! & 
\!\!\!$l$\!\!\! & 
\!\!\!$h$\!\!\! & 
\!\!\!$-$\!\!\! & 
\!\!\!$+$\!\!\! &
$\{  \}$/$\{ t, \textit{\textbf{p}} \}$ &
\!\!\!$\{  \}$/$\{ \textit{\textbf{w}}, t, \textit{\textbf{r}} \}$\!\!\! &
$\{ p \}$/$\{ t \}$ &
$\{ w, r \}$/$\{  \}$ \\
%
\!\!\!$m$\!\!\! & 
\!\!\!$l$\!\!\! & 
\!\!\!$h$\!\!\! & 
\!\!\!$-$\!\!\! & 
\!\!\!$-$\!\!\! &
$\{  \}$/$\{ t, \textit{\textbf{p}} \}$ &
$\{ t, \textit{\textbf{r}} \}$/$\{ w \}$ &
$\{ p \}$/$\{ t \}$ &
$\{ t \}$/$\{ w \}$ \\
%
\!\!\!$l$\!\!\! & 
\!\!\!$m$\!\!\! & 
\!\!\!$h$\!\!\! & 
\!\!\!$-$\!\!\! & 
\!\!\!$+$\!\!\! &
$\{  \}$/$\{ t, \textit{\textbf{p}}  \}$ &
\!\!\!\!$\{  \}$/$\{ \textit{\textbf{w}},\textit{\textbf{t}}, \textit{\textbf{r}} \}$\!\!\!\! &
$\{ p \}$/$\{ t \}$ &
\!\!\!$\{ r \}$/$\{ w, t \}$\!\!\! \\
%
\!\!\!$m$\!\!\! & 
\!\!\!$m$\!\!\! & 
\!\!\!$h$\!\!\! & 
\!\!\!$-$\!\!\! & 
\!\!\!$+$\!\!\! &
$\{ \}$/$\{ t, \textit{\textbf{p}} \}$ &
\!\!\!$\{ w \}$/$\{  \textit{\textbf{t}}, \textit{\textbf{r}} \}$\!\!\! &
$\{ p \}$/$\{ t \}$ &
$\{ t, r \}$/$\{  \}$ \\
%
\!\!\!$h$\!\!\! & 
\!\!\!$l$\!\!\! & 
\!\!\!$h$\!\!\! & 
\!\!\!$-$\!\!\! & 
\!\!\!$-$\!\!\! &
$\{  \}$/$\{ t, \textit{\textbf{p}} \}$ &
\!\!\!$\{ t, \textit{\textbf{r}} \}$/$\{ w \}$\!\!\! &
$\{ p \}$/$\{ t \}$ &
$\{ t \}$/$\{ w \}$ \\
%
\!\!\!$l$\!\!\! & 
\!\!\!$h$\!\!\! & 
\!\!\!$h$\!\!\! & 
\!\!\!$+$\!\!\! & 
\!\!\!$-$\!\!\! &
$\{ \textit{\textbf{p}} \}$/$\{ \textit{\textbf{t}} \}$ &
$\{ \textit{\textbf{w}} \}$/$\{ \textit{\textbf{t}}, \textit{\textbf{r}} \}$ &
$\{ t \}$/$\{  \}$ &
$\{  \}$/$\{ r \}$ \\
%
\!\!\!$h$\!\!\! & 
\!\!\!$m$\!\!\! & 
\!\!\!$h$\!\!\! & 
\!\!\!$-$\!\!\! & 
\!\!\!$+$\!\!\! &
$\{  \}$/$\{ t, \textit{\textbf{p}} \}$ &
$\{ w \}$/$\{ \textit{\textbf{t}}, \textit{\textbf{r}} \}$ &
$\{ p \}$/$\{ t \}$ &
$\{ t, r \}$/$\{  \}$ \\
%
\!\!\!$m$\!\!\! & 
\!\!\!$h$\!\!\! & 
\!\!\!$h$\!\!\! & 
\!\!\!$+$\!\!\! & 
\!\!\!$-$\!\!\! &
$\{ \textit{\textbf{p}} \}$/$\{ \textit{\textbf{t}} \}$ &
\!\!\!$\{  \}$/$\{ w, \textit{\textbf{t}}, \textit{\textbf{r}} \}$\!\!\! &
$\{ t \}$/$\{  \}$ &
$\{  \}$/$\{ w, r \}$ \\
%
\!\!\!$h$\!\!\! & 
\!\!\!$h$\!\!\! & 
\!\!\!$h$\!\!\! & 
\!\!\!$+$\!\!\! & 
\!\!\!$-$\!\!\! &
$\{ \textit{\textbf{p}} \}$/$\{ \textit{\textbf{t}} \}$ &
\!\!\!$\{  \}$/$\{ w, \textit{\textbf{t}},\textit{\textbf{r}} \}$\!\!\! &
$\{ t \}$/$\{  \}$ &
$\{  \}$/$\{ w, r \}$ \\
%
\hline
\end{tabular}

\textbf{\textit{}}

==> 2020 - ArXiv - IDX/tables/overlap.tex <==



\begin{tabular}{r|cc|cc|cc|cc}
\multirow{2}{*}{Dataset} &     
\multicolumn{2}{c}{MD-/LIME-IDX} &   
\multicolumn{2}{c}{MD-/SHAP-IDX} &
\multicolumn{2}{c}{SD-/LIME-IDX} &  
\multicolumn{2}{c}{MD-/SHAP-IDX} \\
                         &  
                         \!\!Agree\!\!  &
                         \!\!Disagree\!\!  &
                         \!\!Agree\!\!  &
                         \!\!Disagree\!\!  &
                         \!\!Agree\!\!  &
                         \!\!Disagree\!\!  &
                         \!\!Agree\!\!  &
                         \!\!Disagree\!\!  \\
\hline
\textbf{Shuttle}  & 
\!\!82.4\%\!\! & 
\!\!17.6\%\!\! & 
\!\!83.6\%\!\! & 
\!\!16.4\%\!\! &
\!\!98.8\%\!\! &  
\!\!1.2\%\!\! & 
\!\!97.1\%\!\! &  
\!\!2.9\%\!\! \\
\textbf{Votes}    & 
\!\!99.1\%\!\! &  
\!\!0.9\%\!\! & 
\!\!78.8\%\!\! & 
\!\!21.2\%\!\! &
\!\!99.1\%\!\! &  
\!\!0.9\%\!\! & 
\!\!78.8\%\!\! & 
\!\!21.2\%\!\! \\
\textbf{Parole}   & 
\!\!65.8\%\!\! & 
\!\!34.2\%\!\! & 
\!\!65.8\%\!\! & 
\!\!34.2\%\!\! &
\!\!91.1\%\!\! &  
\!\!8.9\%\!\! & 
\!\!94.9\%\!\! &  
\!\!5.1\%\!\! \\
\textbf{German}   & 
\!\!50.1\%\!\! & 
\!\!49.9\%\!\! & 
\!\!38.2\%\!\! & 
\!\!61.8\%\!\! &
\!\!83.6\%\!\! & 
\!\!16.4\%\!\! & 
\!\!73.5\%\!\! & 
\!\!26.5\%\!\! \\
\textbf{COMPAS}   & 
\!\!65.7\%\!\! & 
\!\!34.3\%\!\! & 
\!\!20.4\%\!\! & 
\!\!79.6\%\!\! &
\!\!98.3\%\!\! &  
\!\!1.7\%\!\! & 
\!\!54.1\%\!\! & 
\!\!45.9\%\!\! \\
\textbf{Car}      & 
\!\!59.1\%\!\! & 
\!\!40.9\%\!\! & 
\!\!60.3\%\!\! & 
\!\!39.7\%\!\! &
\!\!94.7\%\!\! &  
\!\!5.3\%\!\! & 
\!\!97.1\%\!\! &  
\!\!2.9\%\!\! \\
\textbf{Emotions} & 
\!\!15.0\%\!\! & 
\!\!85.0\%\!\! & 
\!\!12.3\%\!\! & 
\!\!87.7\%\!\! &
\!\!65.0\%\!\! & 
\!\!35.0\%\!\! & 
\!\!51.9\%\!\! & 
\!\!48.1\%\!\! \\
\textbf{Child}    &  
\!\!8.3\%\!\! & 
\!\!91.7\%\!\! &  
\!\!8.3\%\!\! & 
\!\!91.7\%\!\! &
\!\!9.2\%\!\! & 
\!\!90.8\%\!\! &  
\!\!9.3\%\!\! & 
\!\!90.7\%\!\! \\
\textbf{Asia}     & 
\!\!25.0\%\!\! & 
\!\!75.0\%\!\! & 
\!\!25.0\%\!\! & 
\!\!75.0\%\!\! &
\!\!25.0\%\!\! & 
\!\!75.0\%\!\! & 
\!\!25.0\%\!\! & 
\!\!75.0\%\!\! 
\end{tabular}







% OLD (TWO TABLES)


\iffalse
\begin{tabular}{r|cc|cc}
\multirow{2}{*}{Dataset} &     \multicolumn{2}{c}{MD-/LIME-IDX} &   \multicolumn{2}{c}{MD-/SHAP-IDX} \\
                         &  
                         \!\!Agree\!\!  &
                         \!\!Disagree\!\!  &
                         \!\!Agree\!\!  &
                         \!\!Disagree\!\!  \\
\hline
\textbf{Shuttle}  & \!\!82.4\%\!\! & \!\!17.6\%\!\! & \!\!83.6\%\!\! & \!\!16.4\%\!\! \\
\textbf{Votes}    & \!\!99.1\%\!\! &  \!\!0.9\%\!\! & \!\!78.8\%\!\! & \!\!21.2\%\!\! \\
\textbf{Parole}   & \!\!65.8\%\!\! & \!\!34.2\%\!\! & \!\!65.8\%\!\! & \!\!34.2\%\!\! \\
\textbf{German}   & \!\!50.1\%\!\! & \!\!49.9\%\!\! & \!\!38.2\%\!\! & \!\!61.8\%\!\! \\
\textbf{COMPAS}   & \!\!65.7\%\!\! & \!\!34.3\%\!\! & \!\!20.4\%\!\! & \!\!79.6\%\!\! \\
\textbf{Car}      & \!\!59.1\%\!\! & \!\!40.9\%\!\! & \!\!60.3\%\!\! & \!\!39.7\%\!\! \\
\textbf{Emotions} & \!\!15.0\%\!\! & \!\!85.0\%\!\! & \!\!12.3\%\!\! & \!\!87.7\%\!\! \\
\textbf{Child}    &  \!\!8.3\%\!\! & \!\!91.7\%\!\! &  \!\!8.3\%\!\! & \!\!91.7\%\!\! \\
\textbf{Asia}     & \!\!25.0\%\!\! & \!\!75.0\%\!\! & \!\!25.0\%\!\! & \!\!75.0\%\!\! \\
\end{tabular}
\vspace{5mm}\\
\begin{tabular}{r|cc|cc}
\multirow{2}{*}{Dataset} &     \multicolumn{2}{c}{SD-/LIME-IDX} &   \multicolumn{2}{c}{SD-/SHAP-IDX} \\
                         &  
                         \!\!Agree\!\!  &
                         \!\!Disagree\!\!  &
                         \!\!Agree\!\!  &
                         \!\!Disagree\!\!  \\
\hline
\textbf{Shuttle}  & \!\!98.8\%\!\! &  \!\!1.2\%\!\! & \!\!97.1\%\!\! &  \!\!2.9\%\!\! \\
\textbf{Votes}    & \!\!99.1\%\!\! &  \!\!0.9\%\!\! & \!\!78.8\%\!\! & \!\!21.2\%\!\! \\
\textbf{Parole}   & \!\!91.1\%\!\! &  \!\!8.9\%\!\! & \!\!94.9\%\!\! &  \!\!5.1\%\!\! \\
\textbf{German}   & \!\!83.6\%\!\! & \!\!16.4\%\!\! & \!\!73.5\%\!\! & \!\!26.5\%\!\! \\
\textbf{COMPAS}   & \!\!98.3\%\!\! &  \!\!1.7\%\!\! & \!\!54.1\%\!\! & \!\!45.9\%\!\! \\
\textbf{Car}      & \!\!94.7\%\!\! &  \!\!5.3\%\!\! & \!\!97.1\%\!\! &  \!\!2.9\%\!\! \\
\textbf{Emotions} & \!\!65.0\%\!\! & \!\!35.0\%\!\! & \!\!51.9\%\!\! & \!\!48.1\%\!\! \\
\textbf{Child}    &  \!\!9.2\%\!\! & \!\!90.8\%\!\! &  \!\!9.3\%\!\! & \!\!90.7\%\!\! \\
\textbf{Asia}     & \!\!25.0\%\!\! & \!\!75.0\%\!\! & \!\!25.0\%\!\! & \!\!75.0\%\!\! \\
\end{tabular}

\fi

==> 2020 - ArXiv - IDX/tables/play_probs.tex <==
\begin{tabular}{ccccccccccccc}
\hline
\multicolumn{1}{c}{} & 
\!\!\!$w_l$\!\!\! &
\!\!\!$w_m$\!\!\! &
\!\!\!$w_h$\!\!\! &
\!\!\!$t_l$\!\!\! &
\!\!\!$t_m$\!\!\! &
\!\!\!$t_h$\!\!\! &
\!\!\!$p_l$\!\!\! &
\!\!\!$p_h$\!\!\! &
\!\!\!$r_+$\!\!\! &
\!\!\!$r_-$\!\!\! &
\!\!\!$o_+$\!\!\! &
\!\!\!$o_-$\!\!\! \\
\hline
%
\!\!\!$P(\cdot)$\!\!\! & 
\!\!\!$.33$\!\!\! &
\!\!\!$.33$\!\!\! &
\!\!\!$.33$\!\!\! &
\!\!\!$.33$\!\!\! &
\!\!\!$.33$\!\!\! &
\!\!\!$.33$\!\!\! &
\!\!\!$.50$\!\!\! &
\!\!\!$.50$\!\!\! &
\!\!\!$.67$\!\!\! &
\!\!\!$.33$\!\!\! &
\!\!\!$.22$\!\!\! &
\!\!\!$.78$\!\!\! \\
%
\!\!\!$P(\EA{\cdot\, | \,r_+})$\!\!\! & 
$\times$ &
$\times$ &
$\times$ &
\!\!\!$.25$\!\!\! &
\!\!\!$.25$\!\!\! &
\!\!\!$.50$\!\!\! &
\!\!\!$.75$\!\!\! &
\!\!\!$.25$\!\!\! &
$\times$ &
$\times$ &
$\times$ &
$\times$ \\
%
\!\!\!$P(\EA{\cdot\, | \,r_-})$\!\!\! & 
$\times$ &
$\times$ &
$\times$ &
\!\!\!$.49$\!\!\! &
\!\!\!$.49$\!\!\! &
\!\!\!$.02$\!\!\! &
\!\!\!$.02$\!\!\! &
\!\!\!$.98$\!\!\! &
$\times$ &
$\times$ &
$\times$ &
$\times$ \\
%
\!\!\!$P(\EA{\cdot\, | \,o_+})$\!\!\! & 
\!\!\!$.48$\!\!\! &
\!\!\!$.26$\!\!\! &
\!\!\!$.26$\!\!\! &
\!\!\!$.26$\!\!\! &
\!\!\!$.72$\!\!\! &
\!\!\!$.02$\!\!\! &
$\times$ &
$\times$ &
\!\!\!$.02$\!\!\! &
\!\!\!$.98$\!\!\! &
$\times$ &
$\times$ \\
%
\!\!\!$P(\EA{\cdot\, | \,o_-})$\!\!\! & 
\!\!\!$.28$\!\!\! &
\!\!\!$.36$\!\!\! &
\!\!\!$.36$\!\!\! &
\!\!\!$.36$\!\!\! &
\!\!\!$.22$\!\!\! &
\!\!\!$.42$\!\!\! &
$\times$ &
$\times$ &
\!\!\!$.85$\!\!\! &
\!\!\!$.15$\!\!\! &
$\times$ &
$\times$ \\
%
\hline
\end{tabular}

\textbf{\textit{}}

==> 2020 - ArXiv - IDX/tables/play_with_probs.tex <==
\begin{tabular}{ccccccccc}
\hline
	\multicolumn{5}{c}{\!\!$\SF$\!\!} & \multicolumn{2}{c}{SD-\EAB{/\textbf{MD-}}IDX} & %\multicolumn{2}{c}{SD-IDX} & 
	\multicolumn{2}{c}{CF-IDX}  \\
%\cline{1-5}
%\cline{8-8}
\!\!\!$w$\!\!\! & 
\!\!\!$t$\!\!\! & 
%\!\!\!$h$\!\!\! & 
\!\!\!$p$\!\!\! & 
\!\!\!$r$\!\!\! & 
\!\!\!$o$\!\!\! & 
%\!\!$\SDAtts\!(\!r\!)$/$\SDSupps\!(\!r\!)$\!\!\!\! &
\!\!$\dot{-}(\!r\!)$/$\dot{+}(\!r\!)$\!\!\!\! &
\!\!\!$\dot{-}(\!o\!)$/$\dot{+}(\!o\!)$\!\!\! &
\!\!\!$!(\!r\!)$/$*(\!r\!)$\!\!\!\! &
\!\!\!\!$!(\!o\!)$/$*(\!o\!)$\!\!\! \\
\hline
%
\!\!\!$l$\!\!\! & 
\!\!\!$l$\!\!\! & 
\!\!\!$l$\!\!\! & 
\!\!\!$+${\tiny$.94$}\!\!\! & 
\!\!\!$-${\tiny$.99$}\!\!\! &
$\{ t \}$/$\{ \textit{\textbf{p}} \}$ &
$\{ \textit{\textbf{w}} \}$/$\{ t, \textit{\textbf{r}}  \}$ &
$\{ p \}$/$\{  \}$ &
$\{ r \}$/$\{ t \}$ \\
%
\!\!\!$m$\!\!\! & 
\!\!\!$l$\!\!\! & 
\!\!\!$l$\!\!\! & 
\!\!\!$+${\tiny$.94$}\!\!\! & 
\!\!\!$-${\tiny$.99$}\!\!\! &
$\{ t \}$/$\{ \textit{\textbf{p}} \}$ &
\!\!\!$\{  \}$/$\{ w, t, \textit{\textbf{r}} \}$\!\!\! &
$\{ p \}$/$\{  \}$ &
\!\!\!$\{  \}$/$\{ w, t, r \}$\!\!\! \\
%
\!\!\!$l$\!\!\! & 
\!\!\!$m$\!\!\! & 
\!\!\!$l$\!\!\! & 
\!\!\!$+${\tiny$.94$}\!\!\! & 
\!\!\!$-${\tiny$.99$}\!\!\! &
$\{ t \}$/$\{ \textit{\textbf{p}} \}$ &
$\{ \textit{\textbf{w}}, \textit{\textbf{t}} \}$/$\{ \textit{\textbf{r}} \}$ &
$\{ p \}$/$\{  \}$ &
$\{ r \}$/$\{  \}$ \\
%
\!\!\!$m$\!\!\! & 
\!\!\!$m$\!\!\! & 
\!\!\!$l$\!\!\! & 
\!\!\!$+${\tiny$.79$}\!\!\! & 
\!\!\!$-${\tiny$.51$}\!\!\! &
$\{ t \}$/$\{ \textit{\textbf{p}} \}$ &
$\{ \textit{\textbf{t}} \}$/$\{  w, \textit{\textbf{r}} \}$ &
$\{ p \}$/$\{  \}$ &
$\{ r \}$/$\{ w \}$ \\
%
\!\!\!$h$\!\!\! & 
\!\!\!$l$\!\!\! & 
\!\!\!$l$\!\!\! & 
\!\!\!$+${\tiny$.79$}\!\!\! & 
\!\!\!$-${\tiny$.69$}\!\!\! &
$\{ t \}$/$\{ \textit{\textbf{p}} \}$ &
\!\!\!$\{  \}$/$\{ w, t, \textit{\textbf{r}} \}$\!\!\! &
$\{ p \}$/$\{  \}$ &
\!\!\!$\{  \}$/$\{ w, t, r \}$\!\!\! \\
%
\!\!\!$l$\!\!\! & 
\!\!\!$h$\!\!\! & 
\!\!\!$l$\!\!\! & 
\!\!\!$+${\tiny$.79$}\!\!\! & 
\!\!\!$-${\tiny$.51$}\!\!\! &
$\{  \}$/$\{ \textit{\textbf{t}}, \textit{\textbf{p}} \}$ &
$\{ \textit{\textbf{w}} \}$/$\{ \textit{\textbf{t}}, \textit{\textbf{r}} \}$ &
$\{  \}$/$\{ t, p \}$ &
$\{  \}$/$\{ r \}$ \\
%
\!\!\!$h$\!\!\! & 
\!\!\!$m$\!\!\! & 
\!\!\!$l$\!\!\! & 
\!\!\!$+${\tiny$.79$}\!\!\! & 
\!\!\!$-${\tiny$.81$}\!\!\! &
$\{ t \}$/$\{ \textit{\textbf{p}} \}$ &
$\{ \textit{\textbf{t}} \}$/$\{ w, \textit{\textbf{r}} \}$ &
$\{ p \}$/$\{  \}$ &
$\{ r \}$/$\{ w \}$ \\
%
\!\!\!$m$\!\!\! & 
\!\!\!$h$\!\!\! & 
\!\!\!$l$\!\!\! & 
\!\!\!$+${\tiny$.79$}\!\!\! & 
\!\!\!$-${\tiny$.91$}\!\!\! &
$\{  \}$/$\{ \textit{\textbf{t}}, \textit{\textbf{p}} \}$ &
\!\!\!$\{  \}$/$\{ w, \textit{\textbf{t}}, \textit{\textbf{r}} \}$\!\!\! &
$\{  \}$/$\{ t, p \}$ &
$\{  \}$/$\{ w, r \}$ \\
%
\!\!\!$h$\!\!\! & 
\!\!\!$h$\!\!\! & 
\!\!\!$l$\!\!\! & 
\!\!\!$+${\tiny$.79$}\!\!\! & 
\!\!\!$-${\tiny$.81$}\!\!\! &
$\{  \}$/$\{ \textit{\textbf{t}}, \textit{\textbf{p}} \}$ &
\!\!\!$\{  \}$/$\{ w, \textit{\textbf{t}}, \textit{\textbf{r}} \}$\!\!\! &
$\{  \}$/$\{ t, p \}$ &
$\{  \}$/$\{ w, r \}$ \\
%
\!\!\!$l$\!\!\! & 
\!\!\!$l$\!\!\! & 
\!\!\!$h$\!\!\! & 
\!\!\!$-${\tiny$.99$}\!\!\! & 
\!\!\!$+${\tiny$.99$}\!\!\! &
$\{  \}$/$\{ t, \textit{\textbf{p}} \}$ &
\!\!\!$\{  \}$/$\{ \textit{\textbf{w}}, t, \textit{\textbf{r}} \}$\!\!\! &
$\{ p \}$/$\{ t \}$ &
$\{ w, r \}$/$\{  \}$ \\
%
\!\!\!$m$\!\!\! & 
\!\!\!$l$\!\!\! & 
\!\!\!$h$\!\!\! & 
\!\!\!$-${\tiny$.99$}\!\!\! & 
\!\!\!$-${\tiny$.99$}\!\!\! &
$\{  \}$/$\{ t, \textit{\textbf{p}} \}$ &
$\{ t, \textit{\textbf{r}} \}$/$\{ w \}$ &
$\{ p \}$/$\{ t \}$ &
$\{ t \}$/$\{ w \}$ \\
%
\!\!\!$l$\!\!\! & 
\!\!\!$m$\!\!\! & 
\!\!\!$h$\!\!\! & 
\!\!\!$-${\tiny$.99$}\!\!\! & 
\!\!\!$+${\tiny$.99$}\!\!\! &
$\{  \}$/$\{ t, \textit{\textbf{p}}  \}$ &
\!\!\!\!$\{  \}$/$\{ \textit{\textbf{w}},\textit{\textbf{t}}, \textit{\textbf{r}} \}$\!\!\!\! &
$\{ p \}$/$\{ t \}$ &
\!\!\!$\{ r \}$/$\{ w, t \}$\!\!\! \\
%
\!\!\!$m$\!\!\! & 
\!\!\!$m$\!\!\! & 
\!\!\!$h$\!\!\! & 
\!\!\!$-${\tiny$.97$}\!\!\! & 
\!\!\!$+${\tiny$.99$}\!\!\! &
$\{ \}$/$\{ t, \textit{\textbf{p}} \}$ &
\!\!\!$\{ w \}$/$\{  \textit{\textbf{t}}, \textit{\textbf{r}} \}$\!\!\! &
$\{ p \}$/$\{ t \}$ &
$\{ t, r \}$/$\{  \}$ \\
%
\!\!\!$h$\!\!\! & 
\!\!\!$l$\!\!\! & 
\!\!\!$h$\!\!\! & 
\!\!\!$-${\tiny$.97$}\!\!\! & 
\!\!\!$-${\tiny$.99$}\!\!\! &
$\{  \}$/$\{ t, \textit{\textbf{p}} \}$ &
\!\!\!$\{ t, \textit{\textbf{r}} \}$/$\{ w \}$\!\!\! &
$\{ p \}$/$\{ t \}$ &
$\{ t \}$/$\{ w \}$ \\
%
\!\!\!$l$\!\!\! & 
\!\!\!$h$\!\!\! & 
\!\!\!$h$\!\!\! & 
\!\!\!$+${\tiny$.97$}\!\!\! & 
\!\!\!$-${\tiny$.99$}\!\!\! &
$\{ \textit{\textbf{p}} \}$/$\{ \textit{\textbf{t}} \}$ &
$\{ \textit{\textbf{w}} \}$/$\{ \textit{\textbf{t}}, \textit{\textbf{r}} \}$ &
$\{ t \}$/$\{  \}$ &
$\{  \}$/$\{ r \}$ \\
%
\!\!\!$h$\!\!\! & 
\!\!\!$m$\!\!\! & 
\!\!\!$h$\!\!\! & 
\!\!\!$-${\tiny$.97$}\!\!\! & 
\!\!\!$+${\tiny$.98$}\!\!\! &
$\{  \}$/$\{ t, \textit{\textbf{p}} \}$ &
$\{ w \}$/$\{ \textit{\textbf{t}}, \textit{\textbf{r}} \}$ &
$\{ p \}$/$\{ t \}$ &
$\{ t, r \}$/$\{  \}$ \\
%
\!\!\!$m$\!\!\! & 
\!\!\!$h$\!\!\! & 
\!\!\!$h$\!\!\! & 
\!\!\!$+${\tiny$.97$}\!\!\! & 
\!\!\!$-${\tiny$.95$}\!\!\! &
$\{ \textit{\textbf{p}} \}$/$\{ \textit{\textbf{t}} \}$ &
\!\!\!$\{  \}$/$\{ w, \textit{\textbf{t}}, \textit{\textbf{r}} \}$\!\!\! &
$\{ t \}$/$\{  \}$ &
$\{  \}$/$\{ w, r \}$ \\
%
\!\!\!$h$\!\!\! & 
\!\!\!$h$\!\!\! & 
\!\!\!$h$\!\!\! & 
\!\!\!$+${\tiny$.97$}\!\!\! & 
\!\!\!$-${\tiny$.98$}\!\!\! &
$\{ \textit{\textbf{p}} \}$/$\{ \textit{\textbf{t}} \}$ &
\!\!\!$\{  \}$/$\{ w, \textit{\textbf{t}},\textit{\textbf{r}} \}$\!\!\! &
$\{ t \}$/$\{  \}$ &
$\{  \}$/$\{ w, r \}$ \\
%
\hline
\end{tabular}

\textbf{\textit{}}

==> 2020 - ArXiv - IDX/tables/relations_prevalence.tex <==
\begin{tabular}{r|ccc|ccc|ccc|cc|cc}
\multirow{2}{*}{Dataset} & \multicolumn{3}{c}{SD-IDX} & \multicolumn{3}{c}{MD-IDX}  & \multicolumn{3}{c}{CF-IDX} & \multicolumn{2}{c}{LIME-IDX} & \multicolumn{2}{c}{SHAP-IDX}\\
                       & \!\!$\Rels_{\dot{+}}$\!\! & \!\!$\Rels_{\dot{-}}$\!\! & \!\!$\Rels_{\dot{-}\dot{+}}^{\Cla}$\!\! & \!\!$\Rels_{+}$\!\! & \!\!$\Rels_{-}$\!\! & \!\!$\Rels_{-+}^{\Cla}$\!\! & \!\!$\Rels_!$\!\! & \!\!$\Rels_*$\!\! & \!\!$\Rels_{*!}^{\Cla}$\!\! & \!\!$\SuppsLIME$\!\! & \!\!$\AttsLIME$\!\! & \!\!$\SuppsSHAP$\!\! & \!\!$\AttsSHAP$\!\! \\
\hline
  \!\textbf{Shuttle}\! &                 \!59.0\%\! &                 \!41.0\%\! &                            \!$\times$\! &           \!51.2\%\! &           \!32.4\%\! &                \!$\times$\! &         \!17.9\%\! &         \!46.0\%\! &                \!$\times$\! &         \!59.8\%\! &         \!40.2\%\! &         \!61.9\%\! &         \!38.1\%\! \\ 
    \!\textbf{Votes}\! &                 \!77.1\%\! &                 \!22.9\%\! &                            \!$\times$\! &           \!77.1\%\! &           \!22.9\%\! &                \!$\times$\! &          \!3.0\%\! &         \!74.1\%\! &                \!$\times$\! &         \!77.1\%\! &         \!22.9\%\! &         \!73.2\%\! &          \!7.3\%\! \\
   \!\textbf{Parole}\! &                 \!61.5\%\! &                 \!38.5\%\! &                            \!$\times$\! &           \!38.5\%\! &           \!27.4\%\! &                \!$\times$\! &          \!2.1\%\! &         \!70.5\%\! &                \!$\times$\! &         \!55.6\%\! &         \!44.4\%\! &         \!56.4\%\! &         \!43.6\%\! \\
   \!\textbf{German}\! &                 \!59.3\%\! &                 \!40.7\%\! &                            \!$\times$\! &           \!29.6\%\! &           \!22.0\%\! &                \!$\times$\! &      \!$\times$\! &      \!$\times$\! &                \!$\times$\! &         \!55.9\%\! &         \!44.1\%\! &         \!46.9\%\! &         \!36.4\%\! \\
   \!\textbf{COMPAS}\! &                 \!67.0\%\! &                 \!33.0\%\! &                            \!$\times$\! &           \!45.4\%\! &           \!20.3\%\! &                \!$\times$\! &      \!$\times$\! &      \!$\times$\! &                \!$\times$\! &         \!65.7\%\! &         \!34.3\%\! &         \!35.6\%\! &         \!19.1\%\! \\
      \!\textbf{Car}\! &                 \!57.4\%\! &                 \!42.6\%\! &                            \!$\times$\! &           \!39.3\%\! &           \!21.1\%\! &                \!$\times$\! &         \!14.2\%\! &         \!66.4\%\! &                \!$\times$\! &         \!55.3\%\! &         \!44.7\%\! &         \!55.9\%\! &         \!44.1\%\! \\
 \!\textbf{Emotions}\! &                 \!56.9\%\! &                 \!24.0\%\! &                                \!1.1\%\! &           \!10.3\%\! &            \!5.4\%\! &                    \!1.1\%\! &          \!1.9\%\! &          \!1.5\%\! &                \!$\times$\! &         \!60.6\%\! &         \!39.4\%\! &         \!56.8\%\! &         \!10.3\%\! \\
    \!\textbf{Child}\! &                 \!77.5\%\! &                 \!22.5\%\! &                               \!64.0\%\! &           \!65.4\%\! &           \!15.1\%\! &                   \!64.0\%\! &         \!34.6\%\! &         \!27.6\%\! &                   \!64.0\%\! &         \!54.0\%\! &         \!41.3\%\! &         \!24.4\%\! &          \!9.7\%\! \\
     \!\textbf{Asia}\! &                 \!87.5\%\! &                 \!12.5\%\! &                               \!62.5\%\! &           \!87.5\%\! &           \!12.5\%\! &                   \!62.5\%\! &         \!46.9\%\! &          \!9.4\%\! &                   \!62.5\%\! &         \!70.8\%\! &         \!29.2\%\! &         \!54.2\%\! &         \!20.8\%\! \\
\end{tabular}

==> 2020 - ArXiv - IDX/tables/sm_datasets.tex <==
\begin{tabular}{r|cc|cc|cc|cc}
Setting & Data Source$^{*}$  & Classifier Implementation$^{\dagger}$ \\
\hline
\textbf{Shuttle} & DT & \code{skl}\\
\textbf{Parole} & DT & \code{skl}\\
\textbf{German} & DT & \code{skl}\\
\textbf{COMPAS} & DT & \code{skl}\\
\textbf{Car} & DT & \code{skl}\\
\textbf{Emotions} & DT & Chain of \code{skl}\\
\textbf{Asia} & BN & Chain of \code{pgm}\\
\textbf{Child} & BN & Chain of \code{pgm}\\
\end{tabular}

==> tables/old/play.tex <==
\begin{tabular}{ccccccccc}
\hline
	\multicolumn{5}{c}{\!\!$\SF$\!\!} & \multicolumn{2}{c}{SD-IDX} & %\multicolumn{2}{c}{SD-IDX} & 
	\multicolumn{2}{c}{CF-IDX}  \\
%\cline{1-5}
%\cline{8-8}
\!\!\!$w$\!\!\! & 
\!\!\!$t$\!\!\! & 
%\!\!\!$h$\!\!\! & 
\!\!\!$p$\!\!\! & 
\!\!\!$r$\!\!\! & 
\!\!\!$o$\!\!\! & 
%\!\!$\SDAtts\!(\!r\!)$/$\SDSupps\!(\!r\!)$\!\!\!\! &
\!\!$\dot{-}(\!r\!)$/$\dot{+}(\!r\!)$\!\!\!\! &
\!\!\!$\dot{-}(\!o\!)$/$\dot{+}(\!o\!)$\!\!\! &
\!\!\!$!(\!r\!)$/$*(\!r\!)$\!\!\!\! &
\!\!\!\!$!(\!o\!)$/$*(\!o\!)$\!\!\! \\
\hline
%
\!\!\!$l$\!\!\! & 
\!\!\!$l$\!\!\! & 
\!\!\!$l$\!\!\! & 
\!\!\!$+$\!\!\! & 
\!\!\!$-$\!\!\! &
$\{ t \}$/$\{ \textit{\textbf{p}} \}$ &
$\{ \textit{\textbf{w}} \}$/$\{ t, \textit{\textbf{r}}  \}$ &
$\{ p \}$/$\{  \}$ &
$\{ r \}$/$\{ t \}$ \\
%
\!\!\!$m$\!\!\! & 
\!\!\!$l$\!\!\! & 
\!\!\!$l$\!\!\! & 
\!\!\!$+$\!\!\! & 
\!\!\!$-$\!\!\! &
$\{ t \}$/$\{ \textit{\textbf{p}} \}$ &
\!\!\!$\{  \}$/$\{ w, t, \textit{\textbf{r}} \}$\!\!\! &
$\{ p \}$/$\{  \}$ &
\!\!\!$\{  \}$/$\{ w, t, r \}$\!\!\! \\
%
\!\!\!$l$\!\!\! & 
\!\!\!$m$\!\!\! & 
\!\!\!$l$\!\!\! & 
\!\!\!$+$\!\!\! & 
\!\!\!$-$\!\!\! &
$\{ t \}$/$\{ \textit{\textbf{p}} \}$ &
$\{ \textit{\textbf{w}}, \textit{\textbf{t}} \}$/$\{ \textit{\textbf{r}} \}$ &
$\{ p \}$/$\{  \}$ &
$\{ r \}$/$\{  \}$ \\
%
\!\!\!$m$\!\!\! & 
\!\!\!$m$\!\!\! & 
\!\!\!$l$\!\!\! & 
\!\!\!$+$\!\!\! & 
\!\!\!$-$\!\!\! &
$\{ t \}$/$\{ \textit{\textbf{p}} \}$ &
$\{ \textit{\textbf{t}} \}$/$\{  w, \textit{\textbf{r}} \}$ &
$\{ p \}$/$\{  \}$ &
$\{ r \}$/$\{ w \}$ \\
%
\!\!\!$h$\!\!\! & 
\!\!\!$l$\!\!\! & 
\!\!\!$l$\!\!\! & 
\!\!\!$+$\!\!\! & 
\!\!\!$-$\!\!\! &
$\{ t \}$/$\{ \textit{\textbf{p}} \}$ &
\!\!\!$\{  \}$/$\{ w, t, \textit{\textbf{r}} \}$\!\!\! &
$\{ p \}$/$\{  \}$ &
\!\!\!$\{  \}$/$\{ w, t, r \}$\!\!\! \\
%
\!\!\!$l$\!\!\! & 
\!\!\!$h$\!\!\! & 
\!\!\!$l$\!\!\! & 
\!\!\!$+$\!\!\! & 
\!\!\!$-$\!\!\! &
$\{  \}$/$\{ \textit{\textbf{t}}, \textit{\textbf{p}} \}$ &
$\{ \textit{\textbf{w}} \}$/$\{ \textit{\textbf{t}}, \textit{\textbf{r}} \}$ &
$\{  \}$/$\{ t, p \}$ &
$\{  \}$/$\{ r \}$ \\
%
\!\!\!$h$\!\!\! & 
\!\!\!$m$\!\!\! & 
\!\!\!$l$\!\!\! & 
\!\!\!$+$\!\!\! & 
\!\!\!$-$\!\!\! &
$\{ t \}$/$\{ \textit{\textbf{p}} \}$ &
$\{ \textit{\textbf{t}} \}$/$\{ w, \textit{\textbf{r}} \}$ &
$\{ p \}$/$\{  \}$ &
$\{ r \}$/$\{ w \}$ \\
%
\!\!\!$m$\!\!\! & 
\!\!\!$h$\!\!\! & 
\!\!\!$l$\!\!\! & 
\!\!\!$+$\!\!\! & 
\!\!\!$-$\!\!\! &
$\{  \}$/$\{ \textit{\textbf{t}}, \textit{\textbf{p}} \}$ &
\!\!\!$\{  \}$/$\{ w, \textit{\textbf{t}}, \textit{\textbf{r}} \}$\!\!\! &
$\{  \}$/$\{ t, p \}$ &
$\{  \}$/$\{ w, r \}$ \\
%
\!\!\!$h$\!\!\! & 
\!\!\!$h$\!\!\! & 
\!\!\!$l$\!\!\! & 
\!\!\!$+$\!\!\! & 
\!\!\!$-$\!\!\! &
$\{  \}$/$\{ \textit{\textbf{t}}, \textit{\textbf{p}} \}$ &
\!\!\!$\{  \}$/$\{ w, \textit{\textbf{t}}, \textit{\textbf{r}} \}$\!\!\! &
$\{  \}$/$\{ t, p \}$ &
$\{  \}$/$\{ w, r \}$ \\
%
\!\!\!$l$\!\!\! & 
\!\!\!$l$\!\!\! & 
\!\!\!$h$\!\!\! & 
\!\!\!$-$\!\!\! & 
\!\!\!$+$\!\!\! &
$\{  \}$/$\{ t, \textit{\textbf{p}} \}$ &
\!\!\!$\{  \}$/$\{ \textit{\textbf{w}}, t, \textit{\textbf{r}} \}$\!\!\! &
$\{ p \}$/$\{ t \}$ &
$\{ w, r \}$/$\{  \}$ \\
%
\!\!\!$m$\!\!\! & 
\!\!\!$l$\!\!\! & 
\!\!\!$h$\!\!\! & 
\!\!\!$-$\!\!\! & 
\!\!\!$-$\!\!\! &
$\{  \}$/$\{ t, \textit{\textbf{p}} \}$ &
$\{ t, \textit{\textbf{r}} \}$/$\{ w \}$ &
$\{ p \}$/$\{ t \}$ &
$\{ t \}$/$\{ w \}$ \\
%
\!\!\!$l$\!\!\! & 
\!\!\!$m$\!\!\! & 
\!\!\!$h$\!\!\! & 
\!\!\!$-$\!\!\! & 
\!\!\!$+$\!\!\! &
$\{  \}$/$\{ t, \textit{\textbf{p}}  \}$ &
\!\!\!\!$\{  \}$/$\{ \textit{\textbf{w}},\textit{\textbf{t}}, \textit{\textbf{r}} \}$\!\!\!\! &
$\{ p \}$/$\{ t \}$ &
\!\!\!$\{ r \}$/$\{ w, t \}$\!\!\! \\
%
\!\!\!$m$\!\!\! & 
\!\!\!$m$\!\!\! & 
\!\!\!$h$\!\!\! & 
\!\!\!$-$\!\!\! & 
\!\!\!$+$\!\!\! &
$\{ \}$/$\{ t, \textit{\textbf{p}} \}$ &
\!\!\!$\{ w \}$/$\{  \textit{\textbf{t}}, \textit{\textbf{r}} \}$\!\!\! &
$\{ p \}$/$\{ t \}$ &
$\{ t, r \}$/$\{  \}$ \\
%
\!\!\!$h$\!\!\! & 
\!\!\!$l$\!\!\! & 
\!\!\!$h$\!\!\! & 
\!\!\!$-$\!\!\! & 
\!\!\!$-$\!\!\! &
$\{  \}$/$\{ t, \textit{\textbf{p}} \}$ &
\!\!\!$\{ t, \textit{\textbf{r}} \}$/$\{ w \}$\!\!\! &
$\{ p \}$/$\{ t \}$ &
$\{ t \}$/$\{ w \}$ \\
%
\!\!\!$l$\!\!\! & 
\!\!\!$h$\!\!\! & 
\!\!\!$h$\!\!\! & 
\!\!\!$+$\!\!\! & 
\!\!\!$-$\!\!\! &
$\{ \textit{\textbf{p}} \}$/$\{ \textit{\textbf{t}} \}$ &
$\{ \textit{\textbf{w}} \}$/$\{ \textit{\textbf{t}}, \textit{\textbf{r}} \}$ &
$\{ t \}$/$\{  \}$ &
$\{  \}$/$\{ r \}$ \\
%
\!\!\!$h$\!\!\! & 
\!\!\!$m$\!\!\! & 
\!\!\!$h$\!\!\! & 
\!\!\!$-$\!\!\! & 
\!\!\!$+$\!\!\! &
$\{  \}$/$\{ t, \textit{\textbf{p}} \}$ &
$\{ w \}$/$\{ \textit{\textbf{t}}, \textit{\textbf{r}} \}$ &
$\{ p \}$/$\{ t \}$ &
$\{ t, r \}$/$\{  \}$ \\
%
\!\!\!$m$\!\!\! & 
\!\!\!$h$\!\!\! & 
\!\!\!$h$\!\!\! & 
\!\!\!$+$\!\!\! & 
\!\!\!$-$\!\!\! &
$\{ \textit{\textbf{p}} \}$/$\{ \textit{\textbf{t}} \}$ &
\!\!\!$\{  \}$/$\{ w, \textit{\textbf{t}}, \textit{\textbf{r}} \}$\!\!\! &
$\{ t \}$/$\{  \}$ &
$\{  \}$/$\{ w, r \}$ \\
%
\!\!\!$h$\!\!\! & 
\!\!\!$h$\!\!\! & 
\!\!\!$h$\!\!\! & 
\!\!\!$+$\!\!\! & 
\!\!\!$-$\!\!\! &
$\{ \textit{\textbf{p}} \}$/$\{ \textit{\textbf{t}} \}$ &
\!\!\!$\{  \}$/$\{ w, \textit{\textbf{t}},\textit{\textbf{r}} \}$\!\!\! &
$\{ t \}$/$\{  \}$ &
$\{  \}$/$\{ w, r \}$ \\
%
\hline
\end{tabular}

\textbf{\textit{}}
